Dataset Dictionary Learning in a Wasserstein Space for Federated Domain Adaptation

Multi-Source Domain Adaptation (MSDA) is a challenging scenario where multiple related and heterogeneous source datasets must be adapted to an unlabeled target dataset. Conventional MSDA methods often overlook that data holders may have privacy concerns, hindering direct data sharing. In response, decentralized MSDA has emerged as a promising strategy to achieve adaptation without centralizing clients' data. Our work proposes a novel approach, Decentralized Dataset Dictionary Learning, to address this challenge. Our method leverages Wasserstein barycenters to model the distributional shift across multiple clients, enabling effective adaptation while preserving data privacy. Specifically, our algorithm expresses each client's underlying distribution as a Wasserstein barycenter of public atoms, weighted by private barycentric coordinates. Our approach ensures that the barycentric coordinates remain undisclosed throughout the adaptation process. Extensive experimentation across five visual domain adaptation benchmarks demonstrates the superiority of our strategy over existing decentralized MSDA techniques. Moreover, our method exhibits enhanced robustness to client parallelism while maintaining relative resilience compared to conventional decentralized MSDA methodologies.

==> content/fig_distillation.tex <==
\begin{figure}[ht]
    \centering
    \begin{subfigure}{0.32\linewidth}
        \includegraphics[width=\linewidth]{figures/tsne_123.pdf}
        \caption{SPC=$1$}
    \end{subfigure}
    \begin{subfigure}{0.32\linewidth}
        \includegraphics[width=\linewidth]{figures/tsne_1230.pdf}
        \caption{SPC=$10$}
    \end{subfigure}
    \begin{subfigure}{0.32\linewidth}
        \includegraphics[width=\linewidth]{figures/tsne_2460.pdf}
        \caption{SPC=$20$}
    \end{subfigure}\\
    \begin{subfigure}{0.32\linewidth}
        \includegraphics[width=\linewidth]{figures/tsne_entropy_123.pdf}
        \caption{SPC=$1$}
    \end{subfigure}
    \begin{subfigure}{0.32\linewidth}
        \includegraphics[width=\linewidth]{figures/tsne_entropy_1230.pdf}
        \caption{SPC=$10$}
    \end{subfigure}
    \begin{subfigure}{0.32\linewidth}
        \includegraphics[width=\linewidth]{figures/tsne_entropy_2460.pdf}
        \caption{SPC=$20$}
    \end{subfigure}\\
    \begin{subfigure}{0.32\linewidth}
        \includegraphics[width=\linewidth]{figures/entropy_distribution_123.pdf}
        \caption{SPC=$1$}
    \end{subfigure}\hfill
    \begin{subfigure}{0.32\linewidth}
        \includegraphics[width=\linewidth]{figures/entropy_distribution_1230.pdf}
        \caption{SPC=$10$}
    \end{subfigure}\hfill
    \begin{subfigure}{0.32\linewidth}
        \includegraphics[width=\linewidth]{figures/entropy_distribution_2460.pdf}
        \caption{SPC=$20$}
    \end{subfigure}\\
    \begin{subfigure}{0.32\linewidth}
        \includegraphics[width=\linewidth]{figures/Product_Adaptiope_Dataset_Distillation.pdf}
        \caption{Target: Product}
    \end{subfigure}\hfill
    \begin{subfigure}{0.32\linewidth}
        \includegraphics[width=\linewidth]{figures/Real_Adaptiope_Dataset_Distillation.pdf}
        \caption{Target: Real}
    \end{subfigure}\hfill
    \begin{subfigure}{0.32\linewidth}
        \includegraphics[width=\linewidth]{figures/Synthetic_Adaptiope_Dataset_Distillation.pdf}
        \caption{Target: Synthetic}
    \end{subfigure}
    \caption{Dataset distillation on Adaptiope benchmark. (a-c) show a comparison between real (blue) and reconstructed data points (green). (d-f) show the entropy of labels of reconstructed data points. For low values of \gls{spc}, samples have higher label entropy. (g-i) show the distribution of label entropies, in line with the conclusion of (d-f). Finally, (j-l) compares the performance of distillation with samples generated by \gls{dadil}, in comparison to random sub-sampling the source (green) and target (yellow). For \gls{spc}$=5$ (1.67\% of the total amount of samples), one reaches state-of-the-art performance.}
    \label{fig:tsne_reconstruction}
\end{figure}
